Realtime Safety Control for Bipedal Robots to Avoid Multiple Obstacles via CLF-CBF Constraints

This paper presents a reactive planning system that allows a Cassie-series bipedal robot to avoid multiple non-overlapping obstacles via a single, continuously differentiable control barrier function (CBF). The overall system detects an individual obstacle via a height map derived from a LiDAR point cloud and computes an elliptical outer approximation, which is then turned into a CBF. The QP-CLF-CBF formalism developed by Ames et al. is applied to ensure that safe trajectories are generated. Liveness is ensured by an analysis of induced equilibrium points that are distinct from the goal state. Safe planning in environments with multiple obstacles is demonstrated both in simulation and experimentally on the Cassie biped.

==> Archive/Archive1.tex <==
\section{Equilibrium Analysis of Multi-Obstacle Systems}
\label{sec:EquilibriumAnalysis}
\jzl{Single obstacle and Multiple obstacles. Where should we discuss that they are the same for part D}

An equilibrium point of a system is where the optimal control is a zero vector, and thus the robot state remains unchanged. To avoid the undesirable situation, we seek to find equilibrium points $\Ecal = \{x | u^*=[0,0,0]^\transpose, r>0, \text{ and }  \delta,\theta \in (-\pi, \pi] \}$, where $u^*$ is the optimal control variable. Recall that$f=\begin{bmatrix} 0 & 0 & 0 \end{bmatrix}^\transpose$ in \eqref{eq:ControlSystem}, which leads to $L_fV(x)=L_fB(x)=0$. We denote the following to re-write the CLF and the CBF constraints:
\begin{equation}
\label{eq:Aelement}
\begin{aligned}
        % d_x &= -2x_i\cos(\theta)-2y_i\sin(\theta)+2r\cos(\delta) \\
        % d_y &= 2x_i\sin(\theta)-2y_i\cos(\theta)+2r\sin(\delta) \\
        \begin{bmatrix} d_x & d_y & 0 \end{bmatrix} &= -L_gB(x) \\
        \begin{bmatrix} a_x & a_y & a_\omega \end{bmatrix} &= L_gV(x),
\end{aligned}
\end{equation}
where 
\begin{equation}
\label{eq:LgVelement}
\begin{aligned}
        a_x &= -r\cos(\delta) + \frac{\beta\gamma^2\sin(2\beta\delta)  \sin(\delta)}{2r} \\
        a_y &= -r\sin(\delta) - \frac{\beta\gamma^2\sin(2\beta\delta)  \cos(\delta)}{2r} \\
        a_\omega &= \frac{\beta\gamma\sin(2\beta\delta)}{2}.
\end{aligned}
\end{equation}
The constraints become
\begin{align}
    \mathfrak{L}(x,u,s) &= a_xv_x+a_yv_y+a_\omega\omega-s+LLLLV(x),\label{eq:RewriteQPCLFConstraints}\\
    \mathfrak{B}(x,u) &=d_xv_x+d_yv_y-\eta B(x),\label{eq:RewriteQPCBFConstraints}
\end{align}
and the cost function \eqref{eq:QP-cost} of the QP can then be re-written as:
\begin{equation}
\label{eq:RewriteQPCost}
\begin{aligned}
    \mathfrak{J}(u,s)&=\frac{1}{2}h_1(v_x-v_{x}^\mathrm{ref})^2 +\frac{1}{2}h_2(v_y-v_{y}^\mathrm{ref})^2\\
    &+\frac{1}{2}h_3(\omega-\omega^\mathrm{ref})^2+\frac{1}{2}ps^2,
\end{aligned}
\end{equation}
where $\{h_i\}_{i=1}^3$ are the diagonal elements of $H$ in \eqref{eq:QP-cost}, the weights of control variables $[v_x, v_y, \omega]$ with $h_i>0$.

The KKT conditions \cite{gass1997encyclopedia} of this quadratic program are:
\begin{align}
\frac{\partial L}{\partial u}&=Hu^*-Hu^\mathrm{ref}+\mu_1L_gV^\transpose-\mu_2L_gB^\transpose=0 \label{eq:KKT-Stationarity-u} \\
\frac{\partial L}{\partial s}&=ps-\mu_1=0 \label{eq:KKT-Stationarity-s} \\
0&=\mu_1(L_fV+L_gVu^*+LLLLV-s) \label{eq:KKT-slackness-clf} \\
0&=\mu_2(-L_fB-L_gBu^*-\eta B) \label{eq:KKT-slackness-cbf} \\
0 &\geq L_fV+L_gVu^*+LLLLV-s \label{eq:KKT-feasibility-clf} \\
0 &\geq -L_fB-L_gBu^*-\eta B \label{eq:KKT-feasibility-cbf} \\
0 &\leq \mu_1,\mu_2 \label{eq:KKT-dual},
\end{align}
where $\mu_1,\mu_2\in\mathbb{R}$, and $L$ is the Lagrangian function and defined as
\begin{equation}
L(u,s,\mu_1,\mu_2)=\mathfrak{J}(u,s)+\mu_1\mathfrak{L}(x,u,s)+\mu_2\mathfrak{B}(x,u).
\end{equation}

Next, we analyze equilibrium points (if any) via four cases depending on whether each CLF or CBF constraint is active or inactive.
\jzl{The method using KKT conditions is inspired by \cite{LR:Equilibria}}

% Instantly, we know the global minima of \eqref{eq:RewriteQPCost} is achieved by $[u,s] = [v_{x}^\mathrm{ref},v_{y}^\mathrm{ref},\omega^\mathrm{ref},0]$, where $u^\mathrm{ref}$ is the control from the CLF \eqref{eq:CLF} without obstacles, as mentioned in Sec.~\ref{sec:CLF&CBF} and \ref{subsec:QP-of-cbf-clf}. To find $\Ecal$, we consider whether $u^\mathrm{ref}$ fulfills \eqref{eq:QP-clf-constraint} and \eqref{eq:QP-cbf-constraint} and then determine whether $u^*$ is a zero vector. Specifically, we have three cases 
% \begin{equation}
%     \begin{cases}
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})\leq 0, \mathfrak{L}(x,v_x^\mathrm{ref},v_y^\mathrm{ref},\omega^\mathrm{ref},0)\leq 0, \\  
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})\leq 0, \mathfrak{L}(x,v_x^\mathrm{ref},v_y^\mathrm{ref},\omega^\mathrm{ref},0)> 0, \\
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})> 0.
%     \end{cases}
% \end{equation}

% \begin{figure}[t]
% \centering
% \includegraphics[width = 0.45\textwidth]{graphics/dx_dy.png}
% \caption{Illustration showing the geometry meaning of $d_x$ and $d_y$ in the QP constraint. $(d_x,d_y)$ is the position of obstacle center in the robot coordinate.}
% \label{fig:dx_dy}
% \end{figure}

\subsection{Both CLF and CBF are inactive}
\label{subsec:CLF-inactive-CBF-inactive}
When both constraints are inactive, we have 
\begin{equation}
\label{eq:CLF-inactive-CBF-inactive}
\begin{aligned}
    \mu_1&=0\\
    \mu_2&=0\\
    0 &> L_fV+L_gVu^*+LLLLV-s\\
    0 &> -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$ and $s^*$ in this case are
\begin{equation}
\label{eq:CLF-inactive-CBF-inactive-closed}
\begin{aligned}
   u^*&=u^\mathrm{ref} \\
   s^*&=0.
\end{aligned}
\end{equation}
From \eqref{eq:CLFSolution}, as long as the goal is not reached, $u^\mathrm{ref}$ is not a zero vector. Hence, there is no equilibrium point in this case.

\subsection{CLF constraint inactive and CBF constraint active}
\label{subsec:CLF-inactive-CBF-active}
We prove that there is no equilibrium point in this case by contradiction. When the CLF constraint is inactive and the CBF constraint is active, we have 
\begin{equation}
\label{eq:CLF-inactive-CBF-active}
\begin{aligned}
    \mu_1&=0\\
    \mu_2&\geq 0\\
    0 &> L_fV+L_gVu^*+LLLLV-s\\
    0 &= -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$, $s^*$ and $\mu_2$ in this case are
\begin{equation}
\label{eq:CLF-inactive-CBF-active-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} + \mu_2 H^{-1} L_gB^\transpose \\
    s^*&=0\\
    \mu_2 &= -\frac{\eta B + L_fB + L_gBu^\mathrm{ref}}{L_gBH^{-1}L_gB^\transpose}.
\end{aligned}
\end{equation}
If there is an equilibrium point, then $u^*$ is the zero vector. Hence, at the equilibrium point, by $L_fV(x)=0$, $u^*=0$ and $s^*=0$, we have
\begin{equation}
\label{eq:CLF-constraint-CLF-inactive}
L_fV+L_gVu^*+LLLLV-s^* = LLLLV > 0,
\end{equation}
which conflicts with \eqref{eq:CLF-inactive-CBF-active}. Therefore, there is no equilibrium point in this case.

\subsection{CLF constraint active and CBF constraint inactive}
\label{subsec:CLF-active-CBF-inactive}
When the CLF constraint is active and the CBF constraint is inactive, we have 
\begin{equation}
\label{eq:CLF-active-CBF-inactive}
\begin{aligned}
    \mu_1&\geq 0\\
    \mu_2&= 0\\
    0 &= L_fV+L_gVu^*+LLLLV-s\\
    0 &> -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$, $s^*$ and $\mu_1$ in this case are
\begin{equation}
\label{eq:CLF-active-CBF-inactive-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} - \mu_1 H^{-1} L_gV^\transpose \\
    s^*&=\frac{\mu_1}{p}\\
    \mu_1 &= \frac{pLLLLV + pL_fV + pL_gVu^\mathrm{ref}}{pL_gVH^{-1}L_gV^\transpose+1}.
\end{aligned}
\end{equation}
Using the variables defined in \eqref{eq:Aelement}, $u^*$ can be rewritten as:
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\mu_1a_x}{h_1} \\ v_y^\mathrm{ref} - \frac{\mu_1a_y}{h_2} \\ \omega^\mathrm{ref} - \frac{\mu_1a_\omega}{h_3} \end{bmatrix}.
\end{equation}
We know from \eqref{eq:LgVelement} that \jwg{Not sure this true. It depends on $\beta$.}\jzl{In Bruce's paper, $\beta\delta\in[-\pi/2,\pi/2]$. Maybe we should mention that}
\begin{equation}
\label{eq:ay-aomega-delta}
    (a_y=0~~\& ~~a_\omega=0) \Longleftrightarrow \delta=0.
\end{equation}
In addition, we know from \eqref{eq:CLFSolution} that \jwg{Not sure this true. It depends on $\beta$.}
\begin{equation}
\label{eq:vy-omega-delta}
    (v_{y}^\mathrm{ref}=0 ~~\& ~~\omega^\mathrm{ref}=0) \Longleftrightarrow \delta=0.
\end{equation}
Therefore, we split this case into three cases based on the value of $\delta$.

\subsubsection{$\delta=0$ (Case I)} 
\label{subsubsec:CLF-active-CBF-inactive-case1}
Substituting $\delta=0$ to \eqref{eq:Aelement}, we have $a_x=-r<0,a_y=0,a_\omega=0$, and to \eqref{eq:CLFSolution}, we have $v_{x}^\mathrm{ref}>0, v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with \eqref{eq:KKT-dual}, the optimal control command \eqref{eq:CLF-active-CBF-inactive-u} can be simplified as:
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case1}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} + \frac{\mu_1r}{h_1} > 0 \\ 0 \\ 0 \end{bmatrix}.
\end{equation}
The optimal control command is not a zero vector, and hence there is no equilibrium point in this case.

\subsubsection{$\delta>0$ (Case II)} 
\label{subsubsec:CLF-active-CBF-inactive-case2}
When $\delta>0$, by the definitions in \eqref{eq:LgVelement}, we have $a_y<0,a_\omega>0$, and by \eqref{eq:CLFSolution}, we have $v_{y}^\mathrm{ref}>0,\omega^\mathrm{ref}<0$. With \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-inactive-u}, we have
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case2}
\begin{aligned}
v_y^* &= v_y^\mathrm{ref} - \frac{\mu_1a_y}{h_2} > 0\\
\omega^* &= \omega^\mathrm{ref} - \frac{\mu_1a_\omega}{h_3} < 0.
\end{aligned}
\end{equation}
The optimal control command is not a zero vector in this case. Therefore, there is no equilibrium points in this case either.

\subsubsection{$\delta<0$ (Case III)} 
\label{subsubsec:CLF-active-CBF-inactive-case3}
Similarly, by \eqref{eq:Aelement} and \eqref{eq:CLFSolution}, we have $a_y>0,a_\omega<0$ and $v_{y}^\mathrm{ref}<0,\omega^\mathrm{ref}>0$. With \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-inactive-u}, we have
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case3}
\begin{aligned}
v_y^* &= v_y^\mathrm{ref} - \frac{\mu_1a_y}{h_2} < 0\\
\omega^* &= \omega^\mathrm{ref} - \frac{\mu_1a_\omega}{h_3} > 0
\end{aligned}
\end{equation}
The optimal control command is not a zero vector in this case; there is, thus, no equilibrium point in this case.

In summary, there is no equilibrium point when the CLF constraint is active and the CBF constraint is inactive.

\subsection{Both CLF and CBF constraint are active}
\label{subsec:CLF-active-CBF-active}

When the CLF constraint is active and the CBF constraint is active, we have 
\begin{equation}
\label{eq:CLF-active-CBF-active}
\begin{aligned}
    \mu_1&\geq 0\\
    \mu_2&\geq 0\\
    0 &= L_fV+L_gVu^*+LLLLV-s\\
    0 &= -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
We can rewrite \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s} as:
\begin{equation}
\label{eq:CLF-active-CBF-active-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} - \mu_1 H^{-1} L_gV^\transpose + \mu_2 H^{-1} L_gB^\transpose \\
    s^*&=\frac{\mu_1}{p}\\
    % \begin{bmatrix} \mu_1 \\ \mu_2 \end{bmatrix} &= 
    % \begin{bmatrix} 
    %     L_gVH^{-1}L_gV^\transpose+p^{-1} & -L_gVH^{-1}L_gB^\transpose \\ 
    %     L_gBH^{-1}L_gV^\transpose & -L_gBH^{-1}L_gB^\transpose 
    % \end{bmatrix} ^ {-1} 
    % \begin{bmatrix} L_fV + L_gVu^\mathrm{ref}+LLLLV \\ L_fB + L_gBu^\mathrm{ref} + \eta B \end{bmatrix}.
\end{aligned}
\end{equation}
Using the variables defined in \eqref{eq:Aelement}, $u^*$ can be rewritten as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = 
\begin{bmatrix} 
    v_x^\mathrm{ref} - \frac{\mu_1a_x}{h_1} - \frac{\mu_2d_x}{h_1} \\ 
    v_y^\mathrm{ref} - \frac{\mu_1a_y}{h_2} - \frac{\mu_2d_y}{h_2} \\ 
    \omega^\mathrm{ref} - \frac{\mu_1a_\omega}{h_3} 
\end{bmatrix}.
\end{equation}

When the robot is at an equilibrium point, $u^*$ is the zero vector. By \eqref{eq:CLF-active-CBF-active} and $L_fB=0$, $u^*=0$, we have $B=0$, which implies that the robot is at the boundary of an obstacle. In the following proof of Sec. \ref{subsec:CLF-active-CBF-active}, we will assume the robot is at the boundary of obstacles.

The property of $B = 0$ leads to an immediate proposition which is helpful in finding the equilibrium point in the system when one of the components of the optimal control is $0$.
\begin{proposition}
\label{prop:ObstacleBoundary}
$d_y=0 \implies v_x=0$.
\end{proposition}
\begin{proof}
Assume the robot is at the boundary of the $j$th obstacle, we have $\sigma_{\kappa_j} \circ B_j(x)=0$. Since the CBFs $B_i(x)$ are positive distance apart, we have $\sigma_{\kappa_i} \circ B_i(x)>0$ for $\forall i\neq j$. Define $B_{M-1}(x)$ as:
\begin{equation}
    B_{M-1}(x)=\prod_{i}^{i\neq j}\sigma_{\kappa_i} \circ B_i(x).
\end{equation}
We have $B_{M-1}(x)>0$. By the chain rule, the Jacobian of the CBF becomes:
\begin{equation}
\begin{aligned}
        \nabla B_{M}(x)  &=\sigma_{\kappa_j} \circ B_j(x) \frac{\partial B_{M-1}(x)}{\partial x}+B_{M-1}(x) \frac{\partial\sigma_{\kappa_j} \circ B_{j}(x)}{\partial x}\\
                 &= B_{M-1}(x) \left. \frac{d\sigma_{\kappa_j}(s)}{ds} \right|_{s = B_j(x)} \frac{\partial B_{j}(x)}{\partial x} \\
                 &= B_{M-1}(x) \frac{1}{\kappa_j}\frac{\partial B_{j}(x)}{\partial x}.
\end{aligned}
\end{equation}
By $B_{M-1}(x)>0$, $\kappa_j>0$ and $\frac{\partial B_{j}(x)}{\partial x} \neq 0$, we have $\nabla B_M(x) \neq 0$. Since $\mathrm{rank}(g(x))=3$, we have $L_gB(x)=\nabla B(x)\cdot g(x)\neq 0$. Therefore, when $d_y=0$, we have $d_x \neq 0$. With the robot being at the obstacle boundary (i.e., $B=0$), we have $L_gB(x)u=0 \implies v_x=0$. 
\end{proof}

% \begin{figure}[t]
% \centering
% \includegraphics[width = 0.3\textwidth]{graphics/obstacle_boundary.png}
% \caption{Illustration showing the geometry meaning of $d_x$ and $d_y$ when robot is at obstacle boundary. In this condition, $d_x^2+d_y^2=r_o^2$.}
% \label{fig:obstacle_boundary}
% \end{figure}

In addition, with the properties \eqref{eq:ay-aomega-delta} and \eqref{eq:vy-omega-delta}, we split this case into four cases based on whether $\delta$ and $d_y$ are zero.


\subsubsection{$d_y=\delta=0$ (Case I)} 
\label{subsubsec:CLF-active-CBF-active-case1}
Substituting to \eqref{eq:Aelement}, we have $a_x=-r<0,a_y=0,a_\omega=0$, and to \eqref{eq:CLFSolution}, we have $v_{x}^\mathrm{ref}>0,v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with Proposition \ref{prop:ObstacleBoundary}, in this case the optimal control command \eqref{eq:CLF-active-CBF-active-u} can be written as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u-case1}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\mu_1a_x}{h_1} - \frac{\mu_2d_x}{h_1} \\ 0 \\ 0 \end{bmatrix} = \begin{bmatrix} 0 \\ 0 \\ 0 \end{bmatrix}.
\end{equation}
$\mu_1$ and $\mu_2$ can be obtained by \eqref{eq:CLF-active-CBF-active-u-case1}, \eqref{eq:CLF-active-CBF-active} and \eqref{eq:CLF-active-CBF-active-closed}:
\begin{equation}
\label{eq:CLF-active-CBF-active-mu-case1}
\begin{aligned}
\mu_1 &= pLLLLV > 0\\
\mu_2 &= \frac{h_1v_x^\mathrm{ref}-pLLLLVa_x}{d_x}
\end{aligned}
\end{equation}
By \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-active-mu-case1}, we have
\begin{equation}
\label{eq:CLF-active-CBF-active-dx-case1}
\because v_x^\mathrm{ref}>0, a_x<0, \frac{h_1v_x^\mathrm{ref}-pLLLLVa_x}{d_x}\geq0 \longrightarrow d_x>0. 
\end{equation}
Hence, there is an equilibrium point when $B=0$, $d_y=\delta=0$ and $d_x>0$.


\subsubsection{$d_y\neq0,\delta=0$ (Case II)} 
\label{subsubsec:CLF-active-CBF-active-case2}
When $\delta=0$, by \eqref{eq:Aelement} and \eqref{eq:CLFSolution}, we have $a_x=-r<0,a_y=0,a_\omega=0$ and $v_{x}^\mathrm{ref}>0,v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with \eqref{eq:KKT-dual}, the optimal control command \eqref{eq:CLF-active-CBF-active-u} can be simplified as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u-case2}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\mu_1a_x}{h_1} - \frac{\mu_2d_x}{h_1} \\ -\frac{\mu_2d_y}{h_2}\neq0 \\ 0 \end{bmatrix}.
\end{equation}
Because $v_y^*\neq0$, the optimal command is not a zero vector in this case. Equilibrium points don't exist when $d_y\neq$ and $\delta=0$.


\subsubsection{$\delta>0$ (Case III)}
\label{subsubsec:CLF-active-CBF-active-case3}
When $\delta>0$, by \eqref{eq:CLF-active-CBF-inactive-u-case2}, $\omega^*<0$. Hence, the optimal command is not a zero vector and there are no equilibrium points in this case.

\subsubsection{$\delta<0$ (Case IV)} 
\label{subsubsec:CLF-active-CBF-active-case4}
When $\delta<0$, by \eqref{eq:CLF-active-CBF-inactive-u-case3}, $\omega^*>0$. Hence, the optimal command is not a zero vector and there are no equilibrium points in this case.

In summary, the equilibrium point only exists at the obstacle boundary and $\delta=0,d_y=0,d_x>0$ in the four cases.

\begin{figure}[b]
    \centering
    \includegraphics[width = 0.3\textwidth]{equlilibrium1.png}
    \caption{Illustration of an equilibrium case where the robot faces directly to the obstacle and the target. The robot walks back and forth at the obstacle boundary.}
    \label{fig:Equilibrium1}
\end{figure}
 
\subsection{Summary of Equilibrium Points}
In conclusion, the only equilibrium point exits at obstacle boundary and $\delta=0,d_y=0,d_x>0$. At this equilibrium point, the robot faces directly to the obstacle and the target, as shown in Fig.~\ref{fig:Equilibrium1}. The robot will move directly towards the obstacle and stop at the obstacle boundary. 


\begin{figure}[t]
    \centering
    \includegraphics[width = 0.3\textwidth]{equlilibrium2.png}
    \caption{Illustration of breaking the equilibrium by using $u^\mathrm{ref}_2$: $\begin{bmatrix}
        v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} + \epsilon
    \end{bmatrix}^\transpose$ when $\delta=0$. The robot successfully reaches the target position without colliding the obstacle.}
    \label{fig:BreakEquilibrium}
\end{figure}


\subsection{Breaking Equilibrium Points}
When the robot encounters an equilibrium state, we can add a constant $\epsilon$ to $u^\mathrm{ref}$ in \eqref{eq:CBLF-QP} such that $u^\mathrm{ref}=\begin{bmatrix}
        v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} + \epsilon
    \end{bmatrix}^\transpose$,
where $\epsilon = e^{-4}$. As is shown in Fig.~\ref{fig:BreakEquilibrium}, the robot breaks its equilibrium state, avoids the obstacle, and reaches the target position.








==> Archive/Archive2.tex <==
\section{Construction of Control Lyapunov Function and Control Barrier Function}
\label{sec:Methods}
This section introduces the proposed control Lyapunov function and the control barrier function for bipedal robots so that we can ensure the robot is able to smoothly avoid obstacles while account for robot's dynamics.

% To guarantee robot's safety during navigation, we ensure the distance between the robot and the obstacle is always greater than zero.

\subsection{State Representation}
\label{sec:StateRepresentation}
Denote $\Pcal=(x_r,y_r,\theta)$ the robot pose, $\Gcal=(x_t,y_t)$ the goal position in the world frame. We simplify an obstacle $\Ocal$ as a circle (and hence convex) described as its center $(x_o, y_o)$ and its radius $r_o$. We define the robot state as 
\begin{equation}
\label{eq:RobotState}
    x = \begin{bmatrix}
            r \\ 
            \delta\\
            \theta
        \end{bmatrix}, 
\end{equation}
where $r = \sqrt{(x_t-x_r)^2+(y_t-y_r)^2}$, $\theta$ is the heading angle of the robot, and $\delta$ is the angle between $\theta$ and the line of sight from the robot to the goal, as shown in Fig.~\ref{fig:PhysicalMeaning}. 
% \bh{Do we need this? ``The proposed CBF system also contains three dimensional states.'' }

The dynamics of the control system is defined as
\begin{equation}
\label{eq:ControlSystem}
\begin{split}
    \dot{x} &= f(x) + g(x)u \\
    &= 
    \begin{bmatrix}
        0 \\ 
        0 \\
        0
    \end{bmatrix}
    +
    \begin{bmatrix}
        -\cos(\delta) & -\sin(\delta) & 0 \\ 
        \frac{\sin(\delta)}{r} & -\frac{\cos(\delta)}{r} & 1 \\
        0 & 0 & -1
    \end{bmatrix}
    \begin{bmatrix}
        v_x \\ 
        v_y \\
        \omega
    \end{bmatrix},
\end{split}
\end{equation}
where we view $u=\begin{bmatrix} v_x, &v_y, &\omega\end{bmatrix}^\transpose$ as the control variables under the robot frame, as shown in Fig.~\ref{fig:PhysicalMeaning}.

\subsection{Design of CLF and CBF for Bipedal Robots}
\label{sec:CLF&CBF}
The control Lyapunov function leveraged in the reactive planner proposed in \cite{huang2021efficient} takes into account features specific to bipeds, such as the limited lateral leg motion that renders lateral
walking more laborious than sagittal plane walking. Therefore, we also define the CLF as
\begin{equation}
\label{eq:CLF}
    V(x) = \frac{r^2 + \gamma^2\sin^2(\beta\delta)}{2},
\end{equation}
where $\gamma$ is the weight on the orientation, and $\beta$ controls the size of the field of view (FoV). Given $\Pcal$ and $\Gcal$, we have a closed-form solution for control $u$ in \eqref{eq:ControlSystem}, 
\begin{equation}
\label{eq:CLFSolution}
\begin{aligned}
    \omega^\mathrm{ref} &= \frac{r\cos(\delta) \left[ rv_\delta\cos(\delta)-v_r\sin(\delta) \right]}{\alpha + r^2 \cos^2(\delta) }\\
    v_y^\mathrm{ref} &= \frac{\alpha(v_r\sin(\delta)-rv_\delta\cos(\delta))}{r^2{\cos(\delta)}^2+\alpha}\\
    v_x^\mathrm{ref} &= \frac{v_r\cos(\delta)r^2+\alpha v_\delta\sin(\delta)r+\alpha v_r\cos(\delta)}{r^2{\cos(\delta)}^2+\alpha};
\end{aligned}
\end{equation}
where $v_r$ and $v_\delta$ are defined as:
\begin{equation}
\label{eq:feedback}
\begin{aligned}
v_r &= k_{r1}\frac{r}{k_{r2}+r}\\
v_\delta &= -\frac{2}{\beta}k_{\delta 1}\frac{r}{k_{\delta 2}+r}\sin(2\beta\delta).
\end{aligned}
\end{equation}
In \eqref{eq:CLFSolution} and \eqref{eq:feedback}, $\alpha, \beta, k_{r1}, k_{r2}, k_{\delta1}, k_{\delta2}$ are positive constants. See \cite{huang2021efficient} for more details.

Next, we propose the candidate CBF as
\begin{equation}
\label{eq:OriginalCBF}
\begin{aligned}
    B(x) = &(x_{r} - x_o)^2 + (y_{r} - y_o)^2 - r_o^2 \\
         = &(x_{t} - r\cos(\delta+\theta) - x_o)^2 \\ &+ (y_{t} - r\sin(\delta+\theta) - y_o)^2 - r_o^2,
\end{aligned}
\end{equation}
where $(x_o, y_o)$ are the center of an obstacle and $r_o$ is the radius of the obstacle. 
We next verify that \eqref{eq:OriginalCBF} is a valid control barrier function. 

\bh{Yes, we can use the following to be more general.}
\jwg{I think it is no more difficult to use 
$$B(x) := \left[\begin{array}{c} x_{r} - x_o \\ y_{r} - y_o  \end{array}\right]^\top Q  \left[\begin{array}{c} x_{r} - x_o \\ y_{r} - y_o  \end{array} \right] - r_o^2,$$ 
where $Q>0$ and $r_o >0 $. Maybe set $\lambda_{\rm min}(Q) = 1$ ? why does this change nothing? Because later, we'll have $$ a(x) :=  2 \left[ \begin{array}{ll} x_{t} - r\cos(\delta+\theta) - x_o, & y_{t} - r\sin(\delta+\theta) - y_o\end{array} \right] Q $$ and it is still true that $a(x)$ only vanishes at the origin of the obstacle.}

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.45\textwidth]{physical meaning.png}
    \caption{The red line is the distance between the obstacle and the robot.}
    \label{fig:PhysicalMeaning}
\end{figure}



\subsection{Proof of CBF Validity}
\label{subsec:ProofOfCBF}

Following \cite{ames2019control}, we define the sets 
\begin{equation}
    \label{eq:hGreaterThanZero}
    \begin{aligned}
    {\cal D} &:= \{ x \in \real^3~|~ B(x) \neq -r_o^2, \text{ and } r \neq 0\} \\
    {\cal C} & :=\{ x \in {\cal D} ~|~ B(x) \ge 0 \}
    \end{aligned}    
\end{equation}
associated with the candidate CBF \eqref{eq:OriginalCBF} and note that ${\rm Int}(\cal C) \neq \emptyset$ and $\overline{{\rm Int}(\cal C) }= {\cal C}$. From \cite{ames2019control}, for \eqref{eq:OriginalCBF} to be a valid CBF function of \eqref{eq:ControlSystem}, there must exist some $\eta > 0$, such that,
\begin{equation}
\label{eq:CBFrequirement}
\forall x \in {\cal D}, {\exists u \in 
\real^3}, \dot{B}(x,u) +\eta B(x) \geq 0,
\end{equation}
where $\dot{B}(x,u):=L_fB(x) + L_gB(x)u$ is the time derivative of $B(x)$ along the dynamics of  \eqref{eq:ControlSystem}, $\eta>0$ sets the repulsive effort of the CBF, and
\begin{align}
    \label{eq:LieDerivatives}
    L_fB(x) &:= \frac{\partial B(x) }{\partial x} f(x) \\
    L_gB(x) &:= \frac{\partial B(x) }{\partial x} g(x).
\end{align}

Because the drift term $f(x)$ in \eqref{eq:ControlSystem} is identically zero, the zero control $u\equiv 0$ satisfies \eqref{eq:CBFrequirement} for $x \in {\cal C}$. Hence, we need to show that \eqref{eq:CBFrequirement} can be met for $x \in  \thicksim {\cal C}$, the set complement of ${\cal C}$. Direct application of the chain rule gives that $$L_g B(x) = a(x) b(x) g(x),$$ where
\begin{equation}
\label{eq:LgB}
\begin{aligned}
a(x) & :=  2\left[\begin{array}{ll} x_{t} - r\cos(\delta+\theta) - x_o, & y_{t} - r\sin(\delta+\theta) - y_o\end{array}\right]Q \medskip \\
& ~= 2 \left[ \begin{array}{ll}x_r - x_o, &y_r - y_o\end{array} \right] Q \\
    b(x)&:=     \left[ \begin{array}{ccr}
                     -\cos(\delta+\theta) & r\sin(\delta+\theta) & r\sin(\delta+\theta) \\ 
                     -\sin(\delta+\theta) & -r\cos(\delta+\theta) & -r\cos(\delta+\theta) \end{array} \right] \medskip \\ 
 g(x) &~= \left[ \begin{array}{ccr}
                     -\cos(\delta) & -\sin(\delta) & 0 \medskip \\ 
                     \frac{\sin(\delta)}{r} & -\frac{\cos(\delta)}{r} & 1  \medskip\\
                     0 & 0 & -1
                \end{array} \right].
\end{aligned}
\end{equation}
Moreover, $a(x)$ only vanishes at the center of an obstacle, the rows of $b(x)$ are linearly independent for all $r>0$, and 
${\rm det} \left( g(x) \right) = -\frac{1}{r} \neq 0$ for all $0 < r < \infty$. It follows that for all $x \in {\cal D}$, $L_g B(x) \neq 0$ and hence \eqref{eq:CBFrequirement} is satisfied, proving that \eqref{eq:OriginalCBF} is a valid CBF. 



% Because $r\neq 0$ for all $x$ such that the robot has not reached the target


% where $L_pq(x) := \nabla q(x) \cdot p(x)$, which is a derivative operator. 
% With definition of $f(x)$ and $g(x)$ in \eqref{eq:ControlSystem}, $L_fB(x)$ and $L_gB(x)$ becomes
% \begin{equation}
% \label{eq:LieDir}
% \begin{aligned}
%       L_fB(x) &= \nabla B(x) \cdot f(x) \\ &=\nabla B(x) \cdot\begin{bmatrix}
%                 0\\0\\0
%             \end{bmatrix} = 0\\
%       L_gB(x) &= \nabla B(x) g(x) \\ 
%       &= \frac{\partial B}{\partial(x_r, y_r, \theta)} \frac{\partial(x_r, y_r, \theta)}{\partial(r, \delta, \theta)} g(x).
%       % L_gB(x) &= \nabla B(x) \cdot g(x) \\ 
%       % &= \begin{bmatrix} \frac{\partial B}{\partial x_r} & \frac{\partial B}{\partial y_r} & \frac{\partial B}{\partial \theta} \end{bmatrix}     
%       % \begin{bmatrix} 
%       %       \frac{\partial x_r}{\partial r} & \frac{\partial x_r}{\partial \delta} & \frac{\partial x_r}{\partial \theta} \\
%       %       \frac{\partial y_r}{\partial r} & \frac{\partial y_r}{\partial \delta} & \frac{\partial y_r}{\partial \theta} \\
%       %       \frac{\partial \theta}{\partial r} & \frac{\partial \theta}{\partial \delta} & \frac{\partial \theta}{\partial \theta} 
%       % \end{bmatrix} g(x).
% \end{aligned}
% \end{equation}
% Then \eqref{eq:UpdatedCBFRequirement} is true when $B(x)\geq0$ or $L_gB(x)$ is not a zero vector. To analyze when $L_gB(x)$ is a zero vector, we have
% \begin{equation}
% \label{eq:determination}
% \begin{aligned}
% &\det(g(x))=\det\begin{bmatrix}
%                      -\cos(\delta) & -\sin(\delta) & 0 \\ 
%                      \frac{\sin(\delta)}{r} & -\frac{\cos(\delta)}{r} & 1 \\
%                      0 & 0 & -1
%                 \end{bmatrix} = -\frac{1}{r} \neq 0 \\
% &\det\frac{\partial(x_r, y_r, \theta)}{\partial(r, \delta, \theta)}\\ &=
% \det\begin{bmatrix}
%                      -\cos(\delta+\theta) & r\sin(\delta+\theta) & r\sin(\delta+\theta) \\ 
%                      -\sin(\delta+\theta) & -r\cos(\delta+\theta) & -r\cos(\delta+\theta) \\
%                      0 & 0 & 1
%     \end{bmatrix}\\ &= r \neq 0.
% \end{aligned}
% \end{equation}
% From \eqref{eq:LieDir} and \eqref{eq:determination}, we can derive 
% \begin{equation}
% \label{eq:CBF-invalid}
%     L_gB(x)=0 \Longleftrightarrow \frac{\partial B}{\partial(x_r, y_r, \theta)}=0 \Longleftrightarrow \begin{cases} x_r=x_o \\ y_r=y_o \end{cases}.
% \end{equation}
% By \eqref{eq:OriginalCBF}, in this condition, $B(x)=-r_o^2<0$, the requirement \eqref{eq:CBF requirement} can't be satisfied. Therefore, if and only if the robot is not at the center of the obstacle, the CBF function \eqref{eq:OriginalCBF} is valid.



% The Jacobian of the CBF can be readily derived as follows
% \begin{equation}
% \label{eq:Jacobian}
%     \nabla B(x) = 
%     \begin{bmatrix}
%     - 2x_i\cos(\delta+\theta) - 2y_i\sin(\delta+\theta)+2r\\
%     2r(x_i\sin(\delta+\theta)-y_i\cos(\delta+\theta))\\
%     2r(x_i\sin(\delta+\theta)-y_i\cos(\delta+\theta))
%     \end{bmatrix}^\transpose,
% \end{equation}
% where $x_i := x_t - x_o$ and $y_i := y_t - y_o$. Applying \eqref{eq:Jacobian} to \eqref{eq:ControlSystem}, we have
% \begin{equation}
% \label{eq:LieDir}
% \begin{aligned}
%       L_fB(x) &= \nabla B(x) \cdot f(x) \\ &=\nabla B(x) \cdot\begin{bmatrix}
%                 0\\0\\0
%             \end{bmatrix} = 0\\
%       L_gB(x) &= \nabla B(x) \cdot g(x) \\ &=
%         \begin{bmatrix}
%            2x_i\cos(\theta)+2y_i\sin(\theta)-2r\cos(\delta)\\ -2x_i\sin(\theta)+2y_i\cos(\theta)-2r\sin(\delta)\\
%            0
%            \end{bmatrix}^\transpose.      
% \end{aligned}
% \end{equation}

% We then apply \eqref{eq:LieDir} to \eqref{eq:UpdatedCBFRequirement}:
% \begin{equation}
% \begin{aligned}
%     &L_fB(x) + L_gB(x)u + \eta B(x) \\ 
%     &= \begin{bmatrix}
%            2x_i\cos(\theta)+2y_i\sin(\theta)-2r\cos(\delta)\\ -2x_i\sin(\theta)+2y_i\cos(\theta)-2r\sin(\delta)\\
%            0
%            \end{bmatrix}^\transpose \begin{bmatrix}
%               v_x\\ v_y \\ \omega 
%            \end{bmatrix} 
%           +\eta B(x) \\
%     &= v_x \left(2x_i\cos(\theta)+2y_i\sin(\theta)-2r\cos(\delta)\right) \\
%     &+ v_y \left(-2x_i\sin(\theta)+2y_i\cos(\theta)-2r\sin(\delta)\right) \\
%     &+\eta B(x).
% \label{eq:OriginalCBFConstrainsExpression}
% \end{aligned}
% \end{equation}

% When the robot doesn't collide with obstacles, $(x_{r} - x_{o})^2 + (y_{r} - y_{o})^2 > r_{o}^2$. Hence, $B(x)>0$. Then, for $\forall x,\exists u=\begin{bmatrix}
%         0 & 0 & 0
%     \end{bmatrix}^\transpose,\eta>0$, such that $L_fB(x) + L_gB(x)u + \eta B(x) = \eta B(x) > 0$. Therefore, we  prove that the the candidate CBF \eqref{eq:OriginalCBF} is indeed a valid CBF.


\subsection{Quadratic Program of the Proposed CBF-CLF System}
\label{subsec:QP-of-cbf-clf}
A quadratic program (QP) is set up to optimize the control $u$ with the slack variable $s$ while enforcing both the CLF and CBF constraints. Let $\mathfrak{L}(x,u,s)$ be the CLF constrains
\begin{equation}
\label{eq:QP-clf-constraint}
    \mathfrak{L}(x,u,s) := L_fV(x)+L_gV(x)u+LLLLV(x)-s \le 0,
\end{equation}
where $L_pq(x):=\nabla q(x) \cdot p(x)$ is the derivative operator, $\lambda$ serves as a decay rate of the upper bound of $V(x)$. Next, we denote $\mathfrak{B}(x,u)$ the CBF constraints
\begin{equation}
\label{eq:QP-cbf-constraint}
    \mathfrak{B}(x,u) :=-L_fB(x)-L_gB(x)u-\eta B(x) \le 0,
\end{equation}
where $\eta$ serves as a decay rate of the lower bound of $B(x)$.

Finally, the QP for the optimal control is formulated as
\begin{equation}
u^*, s^*=\argmin_{\substack{\mathfrak{L}(x,u,s)\leq 0 \\ \mathfrak{B}(x,u)\leq 0}}\ \mathfrak{J}(u,s),
\label{eq:CBLF-QP}
\end{equation}
where the cost function $\mathfrak{J}(u,s)$ is defined as
\begin{equation}
\label{eq:QP-cost}
    \mathfrak{J}(u,s):=\frac{1}{2}(u-u^\mathrm{ref})^TH(u-u^\mathrm{ref})+\frac{1}{2}ps^2,
\end{equation}
where the positive definite, diagonal matrix $H := {\rm diag}([h_1, h_2, h_3])$ weights the control variables, $u^\mathrm{ref}:=\begin{bmatrix} v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} \end{bmatrix}^\transpose$ is the control from the CLF \eqref{eq:CLF} without obstacles, and $p\ge 0$ is the weight of the slack variable, $s$.


\jwg{Jessy to look at this.} Reference \cite{LR:Equilibria} is our special case where the reference control $u^\mathrm{ref}$ is a zero vector and weight matrix $H$ is an identity matrix. In the proposed CBF-CLF system, $u^\mathrm{ref}$ works as a initial guess obtained from CLF and $H$ assigns weights for different control variables. With these changes, the proposed CBF-CLF system nicely captures inherent features of Cassie-series robots, such as the low-cost of longitudinal movement and high-cost of lateral movement.

% \mathfrak{J}(u,s) is defined as
% \begin{equation}
% \label{eq:QP-cost}
%     \mathfrak{J}(u,s):=(u-u^\mathrm{ref})^TH(u-u^\mathrm{ref})+ps^2,
% \end{equation}
% where the diagonal matrix $H$ weights the control variables, $u^\mathrm{ref}:=\begin{bmatrix} v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} \end{bmatrix}^\transpose$ is the control from the CLF \eqref{eq:CLF} without obstacles, and $p$ is the weight of the slack variable $s$.

% The CLF constraint function is defined as:
% \begin{equation}
% \label{eq:QP-clf-constraint}
%     \mathfrak{L}(x,u,s) := L_fV(x)+L_gV(x)u+LLLLV(x)-s,
% \end{equation}
% where $L_pq(x):=\nabla q(x) \cdot p(x)$ is the derivative operator, $\lambda$ serves as a decay rate of upper bound of $V(x)$.

% We define the cbf constraint function as:
% \begin{equation}
% \label{eq:QP-cbf-constraint}
%     \mathfrak{B}(x,u) :=-L_fB(x)-L_gB(x)u-\eta B(x),
% \end{equation}
% where $\eta$ serves as a decay rate of lower bound of $B(x)$.

% We define the QP of the CBF-CLF as:
% \begin{equation}
% u^*, s^*=\argmin_{\substack{\mathfrak{L}(x,u,s)\leq 0 \\ \mathfrak{B}(x,u)\leq 0}}\ \mathfrak{J}(u,s),
% \label{eq:CBLF-QP}
% \end{equation}
% where the solution $u^*$ is the optimal control command for the robot to follow at the current state, the CLF constraint is $\mathfrak{L}(x,u,s)\leq 0$, the CBF constraint is $\mathfrak{B}(x,u)\leq 0$.


==> Archive/Equilibrium-analysis-multi.tex <==
\section{Equilibrium Analysis of Multi-Obstacle Systems}
\label{sec:EquilibriumAnalysis}


We give the complete analysis for a single obstacle, following the work of \cite{LR:Equilibria}. Because the drift term of our model is zero, any equilibrium points are where the optimal control is the zero vector. To avoid this undesirable situation, we seek to find all equilibrium points $\Ecal = \{x | u^*=[0,0,0]^\transpose, r>0, \text{ and }  \delta,\theta \in (-\pi, \pi] \}$, where $u^*$ is the optimal control variable. Recall that$f=\begin{bmatrix} 0 & 0 & 0 \end{bmatrix}^\transpose$ in \eqref{eq:ControlSystem}, which leads to $L_fV(x)=L_fB(x)=0$. We denote the following to re-write the CLF and the CBF constraints:
\begin{equation}
\label{eq:Aelement}
\begin{aligned}
        % d_x &= -2x_i\cos(\theta)-2y_i\sin(\theta)+2r\cos(\delta) \\
        % d_y &= 2x_i\sin(\theta)-2y_i\cos(\theta)+2r\sin(\delta) \\
        \begin{bmatrix} d_x & d_y & 0 \end{bmatrix} &= -L_gB(x) \\
        \begin{bmatrix} a_x & a_y & a_\omega \end{bmatrix} &= L_gV(x),
\end{aligned}
\end{equation}
where 
\begin{equation}
\label{eq:LgVelement}
\begin{aligned}
        a_x &= -r\cos(\delta) + \frac{\beta\gamma^2\sin(2\beta\delta)  \sin(\delta)}{2r} \\
        a_y &= -r\sin(\delta) - \frac{\beta\gamma^2\sin(2\beta\delta)  \cos(\delta)}{2r} \\
        a_\omega &= \frac{\beta\gamma\sin(2\beta\delta)}{2}.
\end{aligned}
\end{equation}
The constraints become
\begin{align}
    \mathfrak{L}(x,u,s) &= a_xv_x+a_yv_y+a_\omega\omega-s+\mu V(x),\label{eq:RewriteQPCLFConstraints}\\
    \mathfrak{B}(x,u) &=d_xv_x+d_yv_y-\eta B(x),\label{eq:RewriteQPCBFConstraints}
\end{align}
and the cost function \eqref{eq:QP-cost} of the QP can then be re-written as:
\begin{equation}
\label{eq:RewriteQPCost}
\begin{aligned}
    \mathfrak{J}(u,s)&=\frac{1}{2}h_1(v_x-v_{x}^\mathrm{ref})^2 +\frac{1}{2}h_2(v_y-v_{y}^\mathrm{ref})^2\\
    &+\frac{1}{2}h_3(\omega-\omega^\mathrm{ref})^2+\frac{1}{2}ps^2,
\end{aligned}
\end{equation}
where $\{h_i\}_{i=1}^3$ are the diagonal elements of $H$ in \eqref{eq:QP-cost}, the weights of control variables $[v_x, v_y, \omega]$ with $h_i>0$.

The KKT conditions \cite{gass1997encyclopedia} of this quadratic program are:
\begin{align}
\frac{\partial L}{\partial u}&=Hu^*-Hu^\mathrm{ref}+\lambda_1L_gV^\transpose-\lambda_2L_gB^\transpose=0 \label{eq:KKT-Stationarity-u} \\
\frac{\partial L}{\partial s}&=ps-\lambda_1=0 \label{eq:KKT-Stationarity-s} \\
0&=\lambda_1(L_fV+L_gVu^*+\mu V-s) \label{eq:KKT-slackness-clf} \\
0&=\lambda_2(-L_fB-L_gBu^*-\eta B) \label{eq:KKT-slackness-cbf} \\
0 &\geq L_fV+L_gVu^*+\mu V-s \label{eq:KKT-feasibility-clf} \\
0 &\geq -L_fB-L_gBu^*-\eta B \label{eq:KKT-feasibility-cbf} \\
0 &\leq \lambda_1,\lambda_2 \label{eq:KKT-dual},
\end{align}
where $\lambda_1,\lambda_2\in\mathbb{R}$, and $L$ is the Lagrangian function and defined as
\begin{equation}
L(u,s,\lambda_1,\lambda_2)=\mathfrak{J}(u,s)+\lambda_1\mathfrak{L}(x,u,s)+\lambda_2\mathfrak{B}(x,u).
\end{equation}

Next, we analyze equilibrium points (if any) via four cases depending on whether each CLF or CBF constraint is active or inactive following \cite{LR:Equilibria}.

% Instantly, we know the global minima of \eqref{eq:RewriteQPCost} is achieved by $[u,s] = [v_{x}^\mathrm{ref},v_{y}^\mathrm{ref},\omega^\mathrm{ref},0]$, where $u^\mathrm{ref}$ is the control from the CLF \eqref{eq:CLF} without obstacles, as mentioned in Sec.~\ref{sec:CLF&CBF} and \ref{subsec:QP-of-cbf-clf}. To find $\Ecal$, we consider whether $u^\mathrm{ref}$ fulfills \eqref{eq:QP-clf-constraint} and \eqref{eq:QP-cbf-constraint} and then determine whether $u^*$ is a zero vector. Specifically, we have three cases 
% \begin{equation}
%     \begin{cases}
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})\leq 0, \mathfrak{L}(x,v_x^\mathrm{ref},v_y^\mathrm{ref},\omega^\mathrm{ref},0)\leq 0, \\  
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})\leq 0, \mathfrak{L}(x,v_x^\mathrm{ref},v_y^\mathrm{ref},\omega^\mathrm{ref},0)> 0, \\
%     \mathfrak{B}(x,v_{x}^\mathrm{ref},v_{y}^\mathrm{ref})> 0.
%     \end{cases}
% \end{equation}

% \begin{figure}[t]
% \centering
% \includegraphics[width = 0.45\textwidth]{graphics/dx_dy.png}
% \caption{Illustration showing the geometry meaning of $d_x$ and $d_y$ in the QP constraint. $(d_x,d_y)$ is the position of obstacle center in the robot coordinate.}
% \label{fig:dx_dy}
% \end{figure}

\subsection{Both CLF and CBF are inactive}
\label{subsec:CLF-inactive-CBF-inactive}
When both constraints are inactive, we have 
\begin{equation}
\label{eq:CLF-inactive-CBF-inactive}
\begin{aligned}
    \lambda_1&=0\\
    \lambda_2&=0\\
    0 &> L_fV+L_gVu^*+\mu V-s\\
    0 &> -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$ and $s^*$ in this case are
\begin{equation}
\label{eq:CLF-inactive-CBF-inactive-closed}
\begin{aligned}
   u^*&=u^\mathrm{ref} \\
   s^*&=0.
\end{aligned}
\end{equation}
From \eqref{eq:CLFSolution}, as long as the goal is not reached, $u^\mathrm{ref}$ is not a zero vector. Hence, there is no equilibrium point in this case.

\subsection{CLF constraint inactive and CBF constraint active}
\label{subsec:CLF-inactive-CBF-active}
We prove that there is no equilibrium point in this case by contradiction. When the CLF constraint is inactive and the CBF constraint is active, we have 
\begin{equation}
\label{eq:CLF-inactive-CBF-active}
\begin{aligned}
    \lambda_1&=0\\
    \lambda_2&\geq 0\\
    0 &> L_fV+L_gVu^*+\mu V-s\\
    0 &= -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$, $s^*$ and $\lambda_2$ in this case are
\begin{equation}
\label{eq:CLF-inactive-CBF-active-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} + \lambda_2 H^{-1} L_gB^\transpose \\
    s^*&=0\\
    \lambda_2 &= -\frac{\eta B + L_fB + L_gBu^\mathrm{ref}}{L_gBH^{-1}L_gB^\transpose}.
\end{aligned}
\end{equation}
If there is an equilibrium point, then $u^*$ is the zero vector. Hence, at the equilibrium point, by $L_fV(x)=0$, $u^*=0$ and $s^*=0$, we have
\begin{equation}
\label{eq:CLF-constraint-CLF-inactive}
L_fV+L_gVu^*+\mu V-s^* = \mu V > 0,
\end{equation}
which conflicts with \eqref{eq:CLF-inactive-CBF-active}. Therefore, there is no equilibrium point in this case.

\subsection{CLF constraint active and CBF constraint inactive}
\label{subsec:CLF-active-CBF-inactive}
When the CLF constraint is active and the CBF constraint is inactive, we have 
\begin{equation}
\label{eq:CLF-active-CBF-inactive}
\begin{aligned}
    \lambda_1&\geq 0\\
    \lambda_2&= 0\\
    0 &= L_fV+L_gVu^*+\mu V-s\\
    0 &> -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
With \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s}, $u^*$, $s^*$ and $\lambda_1$ in this case are
\begin{equation}
\label{eq:CLF-active-CBF-inactive-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} - \lambda_1 H^{-1} L_gV^\transpose \\
    s^*&=\frac{\lambda_1}{p}\\
    \lambda_1 &= \frac{p\mu V + pL_fV + pL_gVu^\mathrm{ref}}{pL_gVH^{-1}L_gV^\transpose+1}.
\end{aligned}
\end{equation}
Using the variables defined in \eqref{eq:Aelement}, $u^*$ can be rewritten as:
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\lambda_1a_x}{h_1} \\ v_y^\mathrm{ref} - \frac{\lambda_1a_y}{h_2} \\ \omega^\mathrm{ref} - \frac{\lambda_1a_\omega}{h_3} \end{bmatrix}.
\end{equation}
We know from \eqref{eq:LgVelement} that 
% \jwg{Not sure this true. It depends on $\beta$.}\jzl{In Bruce's paper, $\beta\delta\in[-\pi/2,\pi/2]$. Maybe we should mention that}
\begin{equation}
\label{eq:ay-aomega-delta}
    (a_y=0~~\& ~~a_\omega=0) \Longleftrightarrow \delta=0.
\end{equation}
In addition, we know from \eqref{eq:CLFSolution} that 
% \jwg{Not sure this true. It depends on $\beta$.}
\begin{equation}
\label{eq:vy-omega-delta}
    (v_{y}^\mathrm{ref}=0 ~~\& ~~\omega^\mathrm{ref}=0) \Longleftrightarrow \delta=0.
\end{equation}
Therefore, we split this case into three cases based on the value of $\delta$.

\subsubsection{$\delta=0$ (Case I)} 
\label{subsubsec:CLF-active-CBF-inactive-case1}
Substituting $\delta=0$ to \eqref{eq:Aelement}, we have $a_x=-r<0,a_y=0,a_\omega=0$, and to \eqref{eq:CLFSolution}, we have $v_{x}^\mathrm{ref}>0, v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with \eqref{eq:KKT-dual}, the optimal control command \eqref{eq:CLF-active-CBF-inactive-u} can be simplified as:
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case1}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} + \frac{\lambda_1r}{h_1} > 0 \\ 0 \\ 0 \end{bmatrix}.
\end{equation}
The optimal control command is not a zero vector, and hence there is no equilibrium point in this case.

\subsubsection{$\delta>0$ (Case II)} 
\label{subsubsec:CLF-active-CBF-inactive-case2}
When $\delta>0$, by the definitions in \eqref{eq:LgVelement}, we have $a_y<0,a_\omega>0$, and by \eqref{eq:CLFSolution}, we have $v_{y}^\mathrm{ref}>0,\omega^\mathrm{ref}<0$. With \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-inactive-u}, we have
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case2}
\begin{aligned}
v_y^* &= v_y^\mathrm{ref} - \frac{\lambda_1a_y}{h_2} > 0\\
\omega^* &= \omega^\mathrm{ref} - \frac{\lambda_1a_\omega}{h_3} < 0.
\end{aligned}
\end{equation}
The optimal control command is not a zero vector in this case. Therefore, there is no equilibrium points in this case either.

\subsubsection{$\delta<0$ (Case III)} 
\label{subsubsec:CLF-active-CBF-inactive-case3}
Similarly, by \eqref{eq:Aelement} and \eqref{eq:CLFSolution}, we have $a_y>0,a_\omega<0$ and $v_{y}^\mathrm{ref}<0,\omega^\mathrm{ref}>0$. With \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-inactive-u}, we have
\begin{equation}
\label{eq:CLF-active-CBF-inactive-u-case3}
\begin{aligned}
v_y^* &= v_y^\mathrm{ref} - \frac{\lambda_1a_y}{h_2} < 0\\
\omega^* &= \omega^\mathrm{ref} - \frac{\lambda_1a_\omega}{h_3} > 0
\end{aligned}
\end{equation}
The optimal control command is not a zero vector in this case; there is, thus, no equilibrium point in this case.

In summary, there is no equilibrium point when the CLF constraint is active and the CBF constraint is inactive.

\subsection{Both CLF and CBF constraint are active}
\label{subsec:CLF-active-CBF-active}

When the CLF constraint is active and the CBF constraint is active, we have 
\begin{equation}
\label{eq:CLF-active-CBF-active}
\begin{aligned}
    \lambda_1&\geq 0\\
    \lambda_2&\geq 0\\
    0 &= L_fV+L_gVu^*+\mu V-s\\
    0 &= -L_fB-L_gBu^*-\eta B.
\end{aligned}
\end{equation}
We can rewrite \eqref{eq:KKT-Stationarity-u} and \eqref{eq:KKT-Stationarity-s} as:
\begin{equation}
\label{eq:CLF-active-CBF-active-closed}
\begin{aligned}
    u^*&=u^\mathrm{ref} - \lambda_1 H^{-1} L_gV^\transpose + \lambda_2 H^{-1} L_gB^\transpose \\
    s^*&=\frac{\lambda_1}{p}\\
    % \begin{bmatrix} \lambda_1 \\ \lambda_2 \end{bmatrix} &= 
    % \begin{bmatrix} 
    %     L_gVH^{-1}L_gV^\transpose+p^{-1} & -L_gVH^{-1}L_gB^\transpose \\ 
    %     L_gBH^{-1}L_gV^\transpose & -L_gBH^{-1}L_gB^\transpose 
    % \end{bmatrix} ^ {-1} 
    % \begin{bmatrix} L_fV + L_gVu^\mathrm{ref}+\mu V \\ L_fB + L_gBu^\mathrm{ref} + \eta B \end{bmatrix}.
\end{aligned}
\end{equation}
Using the variables defined in \eqref{eq:Aelement}, $u^*$ can be rewritten as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = 
\begin{bmatrix} 
    v_x^\mathrm{ref} - \frac{\lambda_1a_x}{h_1} - \frac{\lambda_2d_x}{h_1} \\ 
    v_y^\mathrm{ref} - \frac{\lambda_1a_y}{h_2} - \frac{\lambda_2d_y}{h_2} \\ 
    \omega^\mathrm{ref} - \frac{\lambda_1a_\omega}{h_3} 
\end{bmatrix}.
\end{equation}

When the robot is at an equilibrium point, $u^*$ is the zero vector. By \eqref{eq:CLF-active-CBF-active} and $L_fB=0$, $u^*=0$, we have $B=0$, which implies that the robot is at the boundary of an obstacle. In the following proof of Sec. \ref{subsec:CLF-active-CBF-active}, we will assume the robot is at the boundary of obstacles.

The property of $B = 0$ leads to an immediate proposition which is helpful in finding the equilibrium point in the system when one of the components of the optimal control is $0$.
\begin{proposition}
\label{prop:ObstacleBoundary}
$d_y=0 \implies v_x=0$.
\end{proposition}
\begin{proof}
Assume the robot is at the boundary of the $j$th obstacle, we have $\sigma_{\kappa_j} \circ B_j(x)=0$. Since the CBFs $B_i(x)$ are positive distance apart, we have $\sigma_{\kappa_i} \circ B_i(x)>0$ for $\forall i\neq j$. Define $B_{M-1}(x)$ as:
\begin{equation}
    B_{M-1}(x)=\prod_{i}^{i\neq j}\sigma_{\kappa_i} \circ B_i(x).
\end{equation}
We have $B_{M-1}(x)>0$. By the chain rule, the Jacobian of the CBF becomes:
\begin{equation}
\begin{aligned}
        \nabla B_{M}(x)  &=\sigma_{\kappa_j} \circ B_j(x) \frac{\partial B_{M-1}(x)}{\partial x}+B_{M-1}(x) \frac{\partial\sigma_{\kappa_j} \circ B_{j}(x)}{\partial x}\\
                 &= B_{M-1}(x) \left. \frac{d\sigma_{\kappa_j}(s)}{ds} \right|_{s = B_j(x)} \frac{\partial B_{j}(x)}{\partial x} \\
                 &= B_{M-1}(x) \frac{1}{\kappa_j}\frac{\partial B_{j}(x)}{\partial x}.
\end{aligned}
\end{equation}
By $B_{M-1}(x)>0$, $\kappa_j>0$ and $\frac{\partial B_{j}(x)}{\partial x} \neq 0$, we have $\nabla B_M(x) \neq 0$. Since $\mathrm{rank}(g(x))=3$, we have $L_gB(x)=\nabla B(x)\cdot g(x)\neq 0$. Therefore, when $d_y=0$, we have $d_x \neq 0$. With the robot being at the obstacle boundary (i.e., $B=0$), we have $L_gB(x)u=0 \implies v_x=0$. 
\end{proof}

% \begin{figure}[t]
% \centering
% \includegraphics[width = 0.3\textwidth]{graphics/obstacle_boundary.png}
% \caption{Illustration showing the geometry meaning of $d_x$ and $d_y$ when robot is at obstacle boundary. In this condition, $d_x^2+d_y^2=r_o^2$.}
% \label{fig:obstacle_boundary}
% \end{figure}

In addition, with the properties \eqref{eq:ay-aomega-delta} and \eqref{eq:vy-omega-delta}, we split this case into four cases based on whether $\delta$ and $d_y$ are zero.


\subsubsection{$d_y=\delta=0$ (Case I)} 
\label{subsubsec:CLF-active-CBF-active-case1}
Substituting to \eqref{eq:Aelement}, we have $a_x=-r<0,a_y=0,a_\omega=0$, and to \eqref{eq:CLFSolution}, we have $v_{x}^\mathrm{ref}>0,v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with Proposition \ref{prop:ObstacleBoundary}, in this case the optimal control command \eqref{eq:CLF-active-CBF-active-u} can be written as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u-case1}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\lambda_1a_x}{h_1} - \frac{\lambda_2d_x}{h_1} \\ 0 \\ 0 \end{bmatrix} = \begin{bmatrix} 0 \\ 0 \\ 0 \end{bmatrix}.
\end{equation}
$\lambda_1$ and $\lambda_2$ can be obtained by \eqref{eq:CLF-active-CBF-active-u-case1}, \eqref{eq:CLF-active-CBF-active} and \eqref{eq:CLF-active-CBF-active-closed}:
\begin{equation}
\label{eq:CLF-active-CBF-active-mu-case1}
\begin{aligned}
\lambda_1 &= p\mu V > 0\\
\lambda_2 &= \frac{h_1v_x^\mathrm{ref}-p\mu Va_x}{d_x}
\end{aligned}
\end{equation}
By \eqref{eq:KKT-dual} and \eqref{eq:CLF-active-CBF-active-mu-case1}, we have
\begin{equation}
\label{eq:CLF-active-CBF-active-dx-case1}
\because v_x^\mathrm{ref}>0, a_x<0, \frac{h_1v_x^\mathrm{ref}-p\mu Va_x}{d_x}\geq0 \longrightarrow d_x>0. 
\end{equation}
Hence, there is an equilibrium point when $B=0$, $d_y=\delta=0$ and $d_x>0$.


\subsubsection{$d_y\neq0,\delta=0$ (Case II)} 
\label{subsubsec:CLF-active-CBF-active-case2}
When $\delta=0$, by \eqref{eq:Aelement} and \eqref{eq:CLFSolution}, we have $a_x=-r<0,a_y=0,a_\omega=0$ and $v_{x}^\mathrm{ref}>0,v_{y}^\mathrm{ref}=0,\omega^\mathrm{ref}=0$. Finally, with \eqref{eq:KKT-dual}, the optimal control command \eqref{eq:CLF-active-CBF-active-u} can be simplified as:
\begin{equation}
\label{eq:CLF-active-CBF-active-u-case2}
u^*=\begin{bmatrix} v_x^* \\ v_y^* \\ \omega^* \end{bmatrix} = \begin{bmatrix} v_x^\mathrm{ref} - \frac{\lambda_1a_x}{h_1} - \frac{\lambda_2d_x}{h_1} \\ -\frac{\lambda_2d_y}{h_2}\neq0 \\ 0 \end{bmatrix}.
\end{equation}
Because $v_y^*\neq0$, the optimal command is not a zero vector in this case. Equilibrium points don't exist when $d_y\neq$ and $\delta=0$.


\subsubsection{$\delta>0$ (Case III)}
\label{subsubsec:CLF-active-CBF-active-case3}
When $\delta>0$, by \eqref{eq:CLF-active-CBF-inactive-u-case2}, $\omega^*<0$. Hence, the optimal command is not a zero vector and there are no equilibrium points in this case.

\subsubsection{$\delta<0$ (Case IV)} 
\label{subsubsec:CLF-active-CBF-active-case4}
When $\delta<0$, by \eqref{eq:CLF-active-CBF-inactive-u-case3}, $\omega^*>0$. Hence, the optimal command is not a zero vector and there are no equilibrium points in this case.

% In summary, the equilibrium point only exists at the obstacle boundary and $\delta=0,d_y=0,d_x>0$ in the four cases.

% \begin{figure}[b]
%     \centering
%     \includegraphics[width = 0.3\textwidth]{equlilibrium1.png}
%     \caption{Illustration of an equilibrium case where the robot faces directly to the obstacle and the target. The robot walks back and forth at the obstacle boundary.}
%     \label{fig:Equilibrium1}
% \end{figure}
 
% \subsection{Summary of Equilibrium Points}
% In conclusion, the only equilibrium point exits at obstacle boundary and $\delta=0,d_y=0,d_x>0$. At this equilibrium point, the robot faces directly to the obstacle and the target, as shown in Fig.~\ref{fig:Equilibrium1}. The robot will move directly towards the obstacle and stop at the obstacle boundary. 


% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 0.3\textwidth]{equlilibrium2.png}
%     \caption{Illustration of breaking the equilibrium by using $u^\mathrm{ref}_2$: $\begin{bmatrix}
%         v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} + \epsilon
%     \end{bmatrix}^\transpose$ when $\delta=0$. The robot successfully reaches the target position without colliding the obstacle.}
%     \label{fig:BreakEquilibrium}
% \end{figure}


% \subsection{Breaking Equilibrium Points}
% When the robot encounters an equilibrium state, we can add a constant $\epsilon$ to $u^\mathrm{ref}$ in \eqref{eq:CBLF-QP} such that $u^\mathrm{ref}=\begin{bmatrix}
%         v_{x}^\mathrm{ref} & v_{y}^\mathrm{ref} & \omega^\mathrm{ref} + \epsilon
%     \end{bmatrix}^\transpose$,
% where $\epsilon = e^{-4}$. As is shown in Fig.~\ref{fig:BreakEquilibrium}, the robot breaks its equilibrium state, avoids the obstacle, and reaches the target position.








==> Archive/Related-Work.tex <==
\section{Related Work}
\label{sec:RelatedWork}
Control barrier functions have become a popular choice in safety-critical navigation problems. In this section, we present related methods and explain the distinction between our work. \jwg{No distinctions are explained. The literature review is not very helpful at present. It does not really explain what is done in the various papers, at least not in a way that I can understand. Please collect 2 or 3 key papers (as PDFs) for each subsection, label them, zip them up, and post them to our slack channel.}

\subsection{Artificial Potential Fields}
An artificial potential field considers a robot as a charged particle and a goal as the opposite charged particle so that the robot can be attracted to the goal \cite{borenstein1989real,hwang1992potential,valavanis2000mobile}. The farther the robot is from the goal, the greater the attraction force. On the other hand, obstacles presented within the environment are the same charge as the robot, which will generate the repelling force to push the robot away from them. In the end, the potential field should be defined everywhere with a force to keep the robot moving toward the goal without colliding with any obstacles.

However, there are local minima issues where attracting fields and repelling field gets superimposed and trap the robot in an unknown state other than the goal. Moreover, oscillating issues happen inside narrow passages or nearby the obstacles. Adaptive potential fields with heuristic functions have been proposed to avoid local minima \cite{IntroLR:PotentialField3,IntroLR:PotentialField4,IntroLR:PF5localminima}. Combining potential fields with gradient functions to reduce oscillating problem is also proposed in \cite{IntroLR:PF6oscillation,IntroLR:PF7oscillation2}. 
Recently, reference \cite{IntroLR:PFvsCBF} demonstrates that a CBF can be considered an advanced potential field method with improved stability for obstacle avoidance tasks.


\subsection{Control Barrier Functions and Control Lyapunov Functions}
Control barrier functions (CBF) have been introduced as a crucial means to provide safety guarantees for nonlinear systems \cite{LR:CBFvsRA, LR:CBFSafety-Critical}. Model Predictive Control (MPC) repeatedly solves constrained finite-horizon nonlinear optimization problems. However, solving such problems in real-time still remains challenging because it is not trivial to predict whether the system will remain within the safe region after applying the control input from the last step \cite{LR:MPClongHorizon1, LR:MPClongHorizon2}. Combining a CBF together with Model Predictive Control (MPC) \cite{LR:CBFMPC1,LR:CBFMPC2,LR:CBFMPC3} enables an MPC-CBF system to take maximum advantage of both approaches. 

% \mzl{\cite{LR:MPClongHorizon1, LR:MPClongHorizon2} (i put the refs, which shows that they need longer horizon to predict for obstacle avoidance cases instead of normal planning.)}


% When single MPC algorithm be applied in collision avoidance tasks, the safety criteria would be added into constrains in the form of Euclidean distance, which results the MPC system will not react unless the robots are close to the obstacles due to the limited prediction horizon range \cite{LR:CBFMPC1,LR:MPC}. Inside the MPC-CBF model, CBF will take charge of safety constrains, which reduce the computational cost on enlarging prediction horizon. 


% \mzl{Reformulating CBF and combining it together with Model Predictive Control (MPC) \cite{LR:CBFMPC1,LR:CBFMPC2,LR:CBFMPC3} enable MPC-CBF system to take the maximum edge from both algorithms.
% When single MPC algorithm be applied in collision avoidance tasks, the safety criteria would be added into constrains in the form of Euclidean distance, which results the MPC system will not react unless the robots are close to the obstacles due to the limited prediction horizon range \cite{LR:CBFMPC1,LR:MPC}. Inside the MPC-CBF model, CBF will take charge of safety constrains, which reduce the computational cost on enlarging prediction horizon.} 


To further improve the robustness of the safety system in practice, managing unknown input disturbance and unmodeled dynamics are proposed in \cite{LR:CBFdisturbance1, LR:CBFdisturbance2,LR:CBFdisturbance3,LR:CBFdisturbance4}. CBFs are also widely used in multi-agent systems for collision avoidance and intersection crossing scenarios \cite{LR:CBF-Multi-Interaction1,LR:CBF-Multi-Interaction2, LR:CBF-Multi-Interaction3, LR:CBF-Multi-Interaction4}. 
Control Lyapunov functions guarantee the stability and convergence for the control system, and have been widely combined with CBFs to address safety-critical problems \cite{LR:CLFsontag1989universal, LR:CBFCLFInsp, LR:CLFCBF1, LR:CLFCBF2, LR:CLFCBF3, LR:CLFCBF4, LR:CLFCBF5, LR:CLFCBF6, LR:CLFCBF7discrete}.
Reference \cite{LR:CLFCBF1} focuses on using CLF-CBF-QP to achieve stable walking for bipedal robots. Applications to solve trajectory planning problems under spatiotemporal and control input constraints are discussed in \cite{LR:CLFCBF4}. Both \cite{LR:CLFCBF2, LR:CLFCBF3} extend their algorithm with point-wise feasibility and asymptotic stability; they, however, still are not able to provide solutions to maintain stability while avoiding obstacles. Moreover, the robot dynamics in \cite{LR:CLFCBF5, LR:CLFCBF6, LR:CLFCBF7discrete} are not applicable to our bipedal robot.

% \mzl{ \cite{LR:CLFCBF7discrete} exploring the bipedal robot walking case in the discrete time domain. and the dynaimic are also different from ours.}
% Also, it is not applicable to fit bipedal dynamic into the robot model in \cite{LR:CLFCBF5, LR:CLFCBF6, LR:CLFCBF7discrete}, which gives the motivation to develop our own CLF-CBF-QP system. An efficient quadratic program (QP) is usually set up to solve the CLF-CBF for real-time applications.

% \mzl{\cite{LR:CLFCBF1} focus on using CLF-CBF-QP to release the stable walking for bipedal robots, and \cite{LR:CLFCBF4} target to solve trajectory planning problem under spatio-temporal, and control input constraints, which are not extendable to our obstacle avoidance problems. Both \cite{LR:CLFCBF2, LR:CLFCBF3} extend the algorithm with point-wise feasibility and symptotic stability, but still not able to provide solution on control bipedal robots conducting safety-critical planning. Also, it is not applicable to fit bipedal dynamic into the robot model in \cite{LR:CLFCBF5, LR:CLFCBF6, LR:CLFCBF7discrete}, which gives the motivation to develop our own CLF-CBF-QP system.}

\subsection{Combining Multiple CBFs for a Control System}

Usually a control barrier function in a control system is designed for a single obstacle. When there are multiple obstacles in the control system, the barrier functions for each obstacle are combined to provide safety guarantees. Reference \cite{rauscher2016constrained} uses multiple CBF constraints for the designed control system. The multiple CBF functions can also be combined to obtain a single CBF function \cite{romdlony2016stabilization, chen2021backup} which can keep robot avoiding obstacles. 

\subsection{CLF-CBF Quadratic Programs and Equilibrium Points}
An equilibrium point of a system is where the robot state remains
unchanged. Reference \cite{LR:Equilibria} shows that although CBF-CLF-QP allows the combination of stability and afwty \jzl{?} in navigation problems, the QP formulation can also lead to undesired equilibrium points in the closed-loop system. With this awareness, \cite{LR:EquilibriaTan} analyzes and proves the existence of equilibrium points in closed-loop systems and demonstrated a modified quadratic program formulation. In addition, \cite{LR:EquilibriaCollisionCone, LR:EquilibriaBall} shows that the unwanted equilibrium point can be removed by transforming the system into a convex manifold, or by increasing the complexity of system states such as including velocities into the system state. 

An equilibrium point is also considered as a ``deadlock'' situation in the multi-agent control system. Reference \cite{LR:EquilibriaMultiAgent} discusses a deadlock scenario with two agents in an one dimensional environment, which is not applicable in our multidimensional system and multi-obstacle environment. 
In addition, \cite{LR:grover2019deadlock} analyze deadlocks for CBF-QP systems where the robot dynamics is assumed as a double-integrator. However, the analysis is still not applicable to our system due to the different robot dynamics.


The present of multiple obstacles is common in practice. Most work applies more CBF constraints to align with the shrink of the safety space \cite{xu2016control,xu2018constrained,LR:multi-CBF}. However, the increasing number of CBF constraints results in high complexity of the QP and quickly become intractable. In this work, we propose a theorem to show that the product of valid CBFs is still a valid CBF for our system, in which we avoid adding CBF constraints so that the complexity of the QP remains constant when the number of obstacles increases.

% The navigation problem for multi-agents is the advanced case of a single agent with multiple obstacles, similar to the previous concept, [Paper 3, 4] considering all other agents as the obstacles and having a CBF constraints inequality for each of the other agents.




% With the increasing application of the CBF-CLF quadratic program (QP) in different kinds of scenarios, researchers are starting to have a deeper understanding of this popular problem solving strategy. \cite{LR:Equilibria} presents that although CBF-CLF QP brings the efficiency and the convenience in navigation type problems, its own QP architecture also creates unwanted equilibrium points in the environment. With this awareness, \cite{LR:EquilibriaTan} analyzed and proved the existence of equilibrium points in closed-loop systems, and demonstrated their modified quadratic program formulation. \cite{LR:EquilibriaCollisionCone, LR:EquilibriaBall} shows that this unwanted equilibrium point can be solved by transforming the system into a convex world, like a ball world, or increasing the complexity of system states, eg. taking the velocity into system state. This equilibrium point can be treated as the deadlock situation in the multi-agent control system. In \cite{LR:EquilibriaMultiAgent}, the research group discusses how gridlock happens with two agents in a one dimensional environment. However, none of them provide the mathematical analysis on more general control affine systems and cannot be applied to analysis our designed system.

% Single obstacle case is always a good start to test the novel navigation algorithm, while the multi-obstacles environment is more common in the real world. To handle this extended scenario,  multiple CBF is introduced into the original QP. Most algorithms, like \cite{xu2016control,xu2018constrained,LR:multi-CBF}, are adding more CBF constraints to align with shrink safety space. However the growing number of CBF constraints will also leads to growing complexity of the calculation, and makes it not suitable for realtime navigation in multiple obstacle environments.
% The navigation problem for multi-agents is the advanced case of a single agent with multiple obstacles, similar to the previous concept, [Paper 3, 4] considering all other agents as the obstacles and having a CBF constraints inequality for each of the other agents.


==> Archive/defines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal packages
\usepackage{bmpsize}
\usepackage{amsthm}
% \usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{amsmath,amssymb,enumerate}
\usepackage{mathrsfs}
\usepackage{times}
\usepackage{multicol}
\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{balance}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dblfloatfix} 
\usepackage{bbold}
\usepackage{makecell}
\usepackage{hhline} % double-line in a table
\usepackage{float} % Places the float at precisely the location in the code
% \usepackage{stfloats} %% float in appendix
% \usepackage{blindtext}

%\usepackage{comment}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{soul} 
% \usepackage{ulem} % Strikethrough in Section Title 
\usepackage{times}
\usepackage{cite}
\usepackage{balance}
\usepackage{dsfont} % indicator function
\usepackage{physics} % partial differential equation
\usepackage{setspace} % double spacing
\usepackage{accents} % widetilde
% \usepackage[style=numeric-comp]{biblatex}

% \usepackage{graphicx}
% \usepackage{fixltx2e}


% packages with options
\usepackage[dvipdfmx]{graphicx} 
\usepackage[T1]{fontenc}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage[utf8]{inputenc}
% \usepackage[title]{appendix}


% packages with setups
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
}

\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
% \let\proof\relax 
% \let\endproof\relax


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Coloring the comment as blue
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Graphics path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{
    {graphics/}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{break}
% \newcounter{exercises}
\newtheorem{assumption}{Assumption}
% \setcounter{assumption}{0}

% \newtheorem{claim}[theorem]{Claim}
\newtheorem{claim}{Claim}

% proof style
\renewcommand\qedsymbol{$\blacksquare$}
\newcommand*{\Qed}{\hfill $\blacksquare$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm inputs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\jad}[1]{[{\textbf{\textcolor{Fuchsia}{Judy: #1}}}]}
\newcommand{\crg}[1]{[{\textbf{\textcolor{Fuchsia}{Craig: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bhdn}[1]{[{\textbf{\textcolor{blue}{Bruce: DATA NEEDED!!#1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhw}[1]{[{\textbf{\textcolor{note}{Bruce: working in progress #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check #1}}}]}
\newcommand{\bhi}[1]{[{\textbf{\textcolor{blue}{Bruce: Illustration only. This figure
will be remade later. #1}}}]}
\newcommand{\bhp}[1]{[{\textbf{\textcolor{blue}{Bruce: Placeholder only. #1}}}]}
\newcommand{\bhm}[1]{[{\textbf{\textcolor{blue}{Bruce: Modified #1}}}]}
\newcommand{\jzl}[1]{[{\textbf{\textcolor{magenta}{Jinze: #1}}}]}
\newcommand{\mzl}[1]{[{\textbf{\textcolor{orange}{Minzhe: #1}}}]}
\definecolor{note}{rgb}{0.3,0.7,0.25}
\definecolor{rephase}{rgb}{0.15,0.7,0.15}
\definecolor{bag}{rgb}{0.5,0.5,0.0}

\newcommand{\add}[1]{\textbf{\textcolor{OliveGreen}{#1}}}
\newcommand{\addd}[1]{{\textcolor{bag}{#1}}}
\newcommand{\mdfy}[2]{\textcolor{Gray}{\st{#1}}\textbf{\textcolor{orange}{#2}}}
\newcommand{\dels}[1]{\textbf{\textcolor{Gray}}{\st{#1}}}
\newcommand{\del}[1]{\textcolor{Gray}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lc}{LiDAR-camera~}
\newcommand{\LC}{LiDAR-Camera~}
\newcommand{\lidar}{LiDAR~}
\newcommand{\lidarNoSpace}{LiDAR}
\newcommand{\lidarN}{LiDAR}
\newcommand{\lidars}{LiDARs~}
\newcommand{\lidarsN}{LiDARs}
\newcommand{\velodyne}{\textit{32-Beam Velodyne ULTRA Puck LiDAR~}}
\newcommand{\velodyneN}{\textit{32-Beam Velodyne ULTRA Puck LiDAR}}
\newcommand{\realsense}{\textit{Intel RealSense Depth Camera D435~}}
\newcommand{\realsenseN}{\textit{Intel RealSense Depth Camera D435}}

\newcommand{\sslidar}{solid-state LiDAR~}
\newcommand{\sslidarN}{solid-state LiDAR}
\newcommand{\sslidars}{solid-state LiDARs~}
\newcommand{\sslidarsN}{solid-state LiDARs}

\newcommand{\slidar}{spinning LiDAR~}
\newcommand{\slidarN}{spinning LiDAR}
\newcommand{\slidars}{spinning LiDARs~}
\newcommand{\slidarsN}{spinning LiDARs}

\newcommand{\lidart}{LiDARTag~}
\newcommand{\lidarts}{LiDARTags~}
\newcommand{\lidartN}{LiDARTag}
\newcommand{\lidartsN}{LiDARTags}

\newcommand{\ltag}{LiDARTag~}
\newcommand{\ltagN}{LiDARTag}
\newcommand{\ltags}{LiDARTags~}
\newcommand{\ltagsN}{LiDARTags}

\newcommand{\atag}{AprilTag~}
\newcommand{\atags}{AprilTags~}
\newcommand{\atagN}{AprilTag}
\newcommand{\atagsN}{AprilTags}

\newcommand{\lind}{linearly independent}
\newcommand{\li}{linearly independent}
\newcommand{\ld}{linearly dependent}

%% Lagrangian Duality
\newcommand{\LanDual}{Lagrangian Duality~}
\newcommand{\LanDualN}{Lagrangian Duality}
\newcommand{\LaDual}{Lagrangian Duality~}
\newcommand{\LaDualN}{Lagrangian Duality}
\newcommand{\LagN}{Lagrangian}
\newcommand{\Lag}{Lagrangian~}
\newcommand{\mm}{Min-Min~}
\newcommand{\mmN}{Min-Min}


% region of interest
\newcommand{\roi}{RoI~}
\newcommand{\rio}{RoI~}
\newcommand{\roiN}{RoI}
\newcommand{\rioN}{RoI}


\newcommand{\pc}{\mathcal{PC}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\BL}{\textbf{BL}}
\newcommand{\bl}{\textbf{BL}}

% coordinates 
\newcommand{\xaxisN}{$x$-axis}
\newcommand{\yaxisN}{$y$-axis}
\newcommand{\zaxisN}{$z$-axis}
\newcommand{\xaxis}{$x$-axis~}
\newcommand{\yaxis}{$y$-axis~}
\newcommand{\zaxis}{$z$-axis~}

% planning 
\newcommand{\Astar}{$\text{A}^*$~}
\newcommand{\AstarN}{$\text{A}^*$}
\newcommand{\Dstar}{$\text{D}^*$~}
\newcommand{\DstarN}{$\text{D}^*$}
\newcommand{\rrt}{$\text{RRT}^*$~}
\newcommand{\rrtN}{$\text{RRT}^*$}
\newcommand{\xobs}{\Xcal_{\text{obs}}}
\newcommand{\xfree}{\Xcal_{\text{free}}}
\newcommand{\traj}{\mathscr{T}}
\newcommand{\nsub}[1]{n_{\text{#1}}}
\newcommand{\csub}[1]{c_{\text{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functionalities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squeezeup}{\vspace{-4mm}} % save space
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\overtilde}[1]{\mkern 1.5mu\widetilde{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\comment}[1]{}

% \long\def\/*#1*/{} % block comments: \/* */



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematics Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\realnumbers{\mathbb{R}}
\def\real{\mathbb{R}}
\def\reals{\mathbb{R}}

\newcommand{\tp}{\mathcal{TP}}
\newcommand{\GPcal}{\mathcal{GP}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\dtheta}{\delta_\theta}
\newcommand{\dphi}{\delta_\phi}
\newcommand{\drho}{\delta_\rho}
\newcommand{\ep}{\mathcal{EP}}
\newcommand{\Pring}{\mathcal{P}}
\newcommand{\plane}{\mathcal{E}}
\newcommand{\vx}{\mathcal{V}}


\newcommand{\indicator}{\mathds{1}}
\newcommand{\EDis}{\mathcal{ED}}
\DeclareDocumentCommand{\RI}{ O{} O{} }{\mathcal{RI}_{#1}^{#2}}
% \newcommand{\RI}{\mathcal{RI}} % region of interest

% operations
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\invv}{\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareDocumentCommand{\td}{ O{} }{\tilde{#1}}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\span}[1]{\left{#1\right}}


% Groups and Algebra
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\Sim}{\mathrm{Sim}}
\newcommand{\Exp}{\mathrm{Exp}}
\newcommand{\Log}{\mathrm{Log}}
%\newcommand{\vect}{\mathrm{vec}}
\newcommand{\vect}[1]{\mathrm{vec}(#1)}
% \newcommand{\Jr}{\mathrm{J_r}}

% Trigonometry
\DeclareDocumentCommand{\asin}{ O{} }{\sin^{-1}(#1)}
\DeclareDocumentCommand{\acos}{ O{} }{\cos^{-1}(#1)}
\DeclareDocumentCommand{\atan}{ O{} }{\tan^{-1}(#1)}


\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}


% \newcommand{\GL}{\mathrm{GL}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}

% \mathbb, mathrm, mathcal, mathsrc, mathop, mathds


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
% \newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


% lowers
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands for letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
\DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
\DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
\DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
\DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
\DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\O}{ O{} O{} }{\textbf{O}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
\DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
\DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
\DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}


% lowers
\DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
\DeclareDocumentCommand{\n}{ O{} O{} }{\textbf{n}_{#1}^{#2}}
\DeclareDocumentCommand{\o}{ O{} O{} }{\textbf{o}_{#1}^{#2}}
\DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
\DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
\DeclareDocumentCommand{\q}{ O{} O{} }{\textbf{q}_{#1}^{#2}}
\DeclareDocumentCommand{\r}{ O{} O{} }{\textbf{r}_{#1}^{#2}}
\DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
\DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}


% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> Archive/newdefine.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal packages
% \usepackage{bmpsize}
\usepackage{amsthm}
% % \usepackage{algorithm, algorithmicx, algpseudocode}
% \usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{amsmath,amssymb,enumerate}
% \usepackage{mathrsfs}
% \usepackage{times}
% \usepackage{multicol}
\usepackage{amsfonts}
% \usepackage{textcomp}
% \usepackage{balance}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{dblfloatfix} 
% \usepackage{bbold}
% \usepackage{makecell}
% \usepackage{hhline} % double-line in a table
% \usepackage{float} % Places the float at precisely the location in the code
% % \usepackage{stfloats} %% float in appendix
% % \usepackage{blindtext}

% %\usepackage{comment}
% \usepackage{xparse}
\usepackage{lipsum}
% \usepackage{soul} 
% % \usepackage{ulem} % Strikethrough in Section Title 
% \usepackage{times}
% \usepackage{cite}
% \usepackage{balance}
% \usepackage{dsfont} % indicator function
% \usepackage{physics} % partial differential equation
% \usepackage{setspace} % double spacing
% \usepackage{accents} % widetilde
% % \usepackage[style=numeric-comp]{biblatex}

% % \usepackage{graphicx}
% % \usepackage{fixltx2e}


% % packages with options
% % \usepackage[dvipdfmx]{graphicx} 
% \usepackage[T1]{fontenc}
% \usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage[caption=false,font=footnotesize]{subfig}
% \usepackage[utf8]{inputenc}
% % \usepackage[title]{appendix}


% % packages with setups
\usepackage{hyperref}
% \hypersetup{
%   colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
% }

% \usepackage{caption}
% \captionsetup{size=footnotesize,
%     %justification=centering, %% not needed
%     skip=5pt, position = bottom}
% % \let\proof\relax 
% % \let\endproof\relax


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Algorithm 
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%% Coloring the comment as blue
% \newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
% \SetCommentSty{mycommfont}

% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Graphics path
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \graphicspath{
%     {graphics/}
% }


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Theorem style
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newtheoremstyle{break}
%   {\topsep}{\topsep}%
%   {\itshape}{}%
%   {\bfseries}{}%
%   {\newline}{}%



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Environments
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

% \theoremstyle{break}
% % \newcounter{exercises}
% \newtheorem{assumption}{Assumption}
% % \setcounter{assumption}{0}

% % \newtheorem{claim}[theorem]{Claim}
% \newtheorem{claim}{Claim}

% % proof style
% \renewcommand\qedsymbol{$\blacksquare$}
% \newcommand*{\Qed}{\hfill $\blacksquare$}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm inputs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\jad}[1]{[{\textbf{\textcolor{Fuchsia}{Judy: #1}}}]}
\newcommand{\crg}[1]{[{\textbf{\textcolor{Fuchsia}{Craig: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bhdn}[1]{[{\textbf{\textcolor{blue}{Bruce: DATA NEEDED!!#1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhw}[1]{[{\textbf{\textcolor{note}{Bruce: working in progress #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check #1}}}]}
\newcommand{\bhi}[1]{[{\textbf{\textcolor{blue}{Bruce: Illustration only. This figure
will be remade later. #1}}}]}
\newcommand{\bhp}[1]{[{\textbf{\textcolor{blue}{Bruce: Placeholder only. #1}}}]}
\newcommand{\bhm}[1]{[{\textbf{\textcolor{blue}{Bruce: Modified #1}}}]}
\newcommand{\jzl}[1]{[{\textbf{\textcolor{magenta}{Jinze: #1}}}]}
\newcommand{\mzl}[1]{[{\textbf{\textcolor{orange}{Minzhe: #1}}}]}
% \definecolor{note}{rgb}{0.3,0.7,0.25}
% \definecolor{rephase}{rgb}{0.15,0.7,0.15}
% \definecolor{bag}{rgb}{0.5,0.5,0.0}

\newcommand{\add}[1]{\textbf{\textcolor{OliveGreen}{#1}}}
\newcommand{\addd}[1]{{\textcolor{bag}{#1}}}
\newcommand{\mdfy}[2]{\textcolor{Gray}{\st{#1}}\textbf{\textcolor{orange}{#2}}}
\newcommand{\dels}[1]{\textbf{\textcolor{Gray}}{\st{#1}}}
\newcommand{\del}[1]{\textcolor{Gray}{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lc}{LiDAR-camera~}
\newcommand{\LC}{LiDAR-Camera~}
\newcommand{\lidar}{LiDAR~}
\newcommand{\lidarNoSpace}{LiDAR}
\newcommand{\lidarN}{LiDAR}
\newcommand{\lidars}{LiDARs~}
\newcommand{\lidarsN}{LiDARs}
\newcommand{\velodyne}{\textit{32-Beam Velodyne ULTRA Puck LiDAR~}}
\newcommand{\velodyneN}{\textit{32-Beam Velodyne ULTRA Puck LiDAR}}
\newcommand{\realsense}{\textit{Intel RealSense Depth Camera D435~}}
\newcommand{\realsenseN}{\textit{Intel RealSense Depth Camera D435}}

\newcommand{\sslidar}{solid-state LiDAR~}
\newcommand{\sslidarN}{solid-state LiDAR}
\newcommand{\sslidars}{solid-state LiDARs~}
\newcommand{\sslidarsN}{solid-state LiDARs}

\newcommand{\slidar}{spinning LiDAR~}
\newcommand{\slidarN}{spinning LiDAR}
\newcommand{\slidars}{spinning LiDARs~}
\newcommand{\slidarsN}{spinning LiDARs}

\newcommand{\lidart}{LiDARTag~}
\newcommand{\lidarts}{LiDARTags~}
\newcommand{\lidartN}{LiDARTag}
\newcommand{\lidartsN}{LiDARTags}

\newcommand{\ltag}{LiDARTag~}
\newcommand{\ltagN}{LiDARTag}
\newcommand{\ltags}{LiDARTags~}
\newcommand{\ltagsN}{LiDARTags}

\newcommand{\atag}{AprilTag~}
\newcommand{\atags}{AprilTags~}
\newcommand{\atagN}{AprilTag}
\newcommand{\atagsN}{AprilTags}

\newcommand{\lind}{linearly independent}
\newcommand{\li}{linearly independent}
\newcommand{\ld}{linearly dependent}

%% Lagrangian Duality
\newcommand{\LanDual}{Lagrangian Duality~}
\newcommand{\LanDualN}{Lagrangian Duality}
\newcommand{\LaDual}{Lagrangian Duality~}
\newcommand{\LaDualN}{Lagrangian Duality}
\newcommand{\LagN}{Lagrangian}
\newcommand{\Lag}{Lagrangian~}
\newcommand{\mm}{Min-Min~}
\newcommand{\mmN}{Min-Min}


% region of interest
\newcommand{\roi}{RoI~}
\newcommand{\rio}{RoI~}
\newcommand{\roiN}{RoI}
\newcommand{\rioN}{RoI}


\newcommand{\pc}{\mathcal{PC}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\BL}{\textbf{BL}}
\newcommand{\bl}{\textbf{BL}}

% coordinates 
\newcommand{\xaxisN}{$x$-axis}
\newcommand{\yaxisN}{$y$-axis}
\newcommand{\zaxisN}{$z$-axis}
\newcommand{\xaxis}{$x$-axis~}
\newcommand{\yaxis}{$y$-axis~}
\newcommand{\zaxis}{$z$-axis~}

% planning 
\newcommand{\Astar}{$\text{A}^*$~}
\newcommand{\AstarN}{$\text{A}^*$}
\newcommand{\Dstar}{$\text{D}^*$~}
\newcommand{\DstarN}{$\text{D}^*$}
\newcommand{\rrt}{$\text{RRT}^*$~}
\newcommand{\rrtN}{$\text{RRT}^*$}
\newcommand{\xobs}{\Xcal_{\text{obs}}}
\newcommand{\xfree}{\Xcal_{\text{free}}}
\newcommand{\traj}{\mathscr{T}}
\newcommand{\nsub}[1]{n_{\text{#1}}}
\newcommand{\csub}[1]{c_{\text{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functionalities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squeezeup}{\vspace{-4mm}} % save space
\newcommand{\overbar}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\overtilde}[1]{\mkern 1.5mu\widetilde{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}
\newcommand{\comment}[1]{}

% \long\def\/*#1*/{} % block comments: \/* */



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematics Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\realnumbers{\mathbb{R}}
\def\real{\mathbb{R}}
\def\reals{\mathbb{R}}

\newcommand{\tp}{\mathcal{TP}}
\newcommand{\GPcal}{\mathcal{GP}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\dtheta}{\delta_\theta}
\newcommand{\dphi}{\delta_\phi}
\newcommand{\drho}{\delta_\rho}
\newcommand{\ep}{\mathcal{EP}}
\newcommand{\Pring}{\mathcal{P}}
\newcommand{\plane}{\mathcal{E}}
\newcommand{\vx}{\mathcal{V}}


\newcommand{\indicator}{\mathds{1}}
\newcommand{\EDis}{\mathcal{ED}}
\DeclareDocumentCommand{\RI}{ O{} O{} }{\mathcal{RI}_{#1}^{#2}}
% \newcommand{\RI}{\mathcal{RI}} % region of interest

% operations
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\invv}{\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareDocumentCommand{\td}{ O{} }{\tilde{#1}}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\span}[1]{\left{#1\right}}


% Groups and Algebra
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\Sim}{\mathrm{Sim}}
\newcommand{\Exp}{\mathrm{Exp}}
\newcommand{\Log}{\mathrm{Log}}
%\newcommand{\vect}{\mathrm{vec}}
\newcommand{\vect}[1]{\mathrm{vec}(#1)}
% \newcommand{\Jr}{\mathrm{J_r}}

% Trigonometry
\DeclareDocumentCommand{\asin}{ O{} }{\sin^{-1}(#1)}
\DeclareDocumentCommand{\acos}{ O{} }{\cos^{-1}(#1)}
\DeclareDocumentCommand{\atan}{ O{} }{\tan^{-1}(#1)}


\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}


% \newcommand{\GL}{\mathrm{GL}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}

% \mathbb, mathrm, mathcal, mathsrc, mathop, mathds


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
% \newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}


% lowers
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands for letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
\DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
\DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
\DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
\DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
\DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\O}{ O{} O{} }{\textbf{O}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
\DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
\DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
\DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}


% lowers
\DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
\DeclareDocumentCommand{\n}{ O{} O{} }{\textbf{n}_{#1}^{#2}}
\DeclareDocumentCommand{\o}{ O{} O{} }{\textbf{o}_{#1}^{#2}}
\DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
\DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
\DeclareDocumentCommand{\q}{ O{} O{} }{\textbf{q}_{#1}^{#2}}
\DeclareDocumentCommand{\r}{ O{} O{} }{\textbf{r}_{#1}^{#2}}
\DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
\DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}


% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> bio.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Bruce.png}}]{Jiunn-Kai Huang} received the PhD degree in robotics from the University of Michigan, Ann Arbor in 2022. His research focused on autonomy of bipedal robots, encompassing sensor fusion, pose estimation, and motion planning. He was in charge of building a full stack of autonomy pipeline for the system integration of Cassie Blue, a bipedal robot with 20 degrees of freedom.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{headshotJWG2.jpg}}]{Jessy W. Grizzle} (S’78–M’83–F’97) received the Ph.D. in electrical engineering from The University of Texas at Austin in 1983. He is a Professor of Robotics at the University of Michigan, where he holds the titles of the Elmer Gilbert Distinguished University Professor and the Jerry and Carol Levin Professor of Engineering. He jointly holds sixteen patents dealing with emissions reduction in passenger vehicles through improved control system design. Professor Grizzle is a Fellow of the IEEE and IFAC. He received the Paper of the Year Award from the IEEE Vehicular Technology Society in 1993, the George S. Axelby Award in 2002, the Control Systems Technology Award in 2003, the Bode Prize in 2012, the IEEE Transactions on Control Systems Technology Outstanding Paper Award in 2014, and the  IEEE Transactions on Automation Science and Engineering, Googol Best New Application Paper Award in 2019. His work on bipedal locomotion has been the object of numerous plenary lectures and has been featured on CNN, ESPN, Discovery Channel, The Economist, Wired Magazine, Discover Magazine, Scientific American and Popular Mechanics.
\end{IEEEbiography}

